Building Proteins in a Day: Efficient 3D Molecular Reconstruction

Discovering the 3D atomic structure of molecules such as proteins and viruses is a fundamental research problem in biology and medicine. Electron Cryomicroscopy (Cryo-EM) is a promising vision-based technique for structure estimation which attempts to reconstruct 3D structures from 2D images. This paper addresses the challenging problem of 3D reconstruction from 2D Cryo-EM images. A new framework for estimation is introduced which relies on modern stochastic optimization techniques to scale to large datasets. We also introduce a novel technique which reduces the cost of evaluating the objective function during optimization by over five orders or magnitude. The net result is an approach capable of estimating 3D molecular structure from large scale datasets in about a day on a single workstation.

==> fig_ctf.tex <==
\begin{figure}
\centering
\includegraphics[width=0.25\textwidth]{figs/ctf2D0.pdf}
\includegraphics[width=0.33\textwidth]{figs/ctf1D0.pdf}
\caption{\label{fig:ctf}
The Contrast Transfer Function (CTF) modulates the integral projection.  Note
that the phase changes and zero crossings make estimation particularly 
challenging.  The specific locations of the zero crossings will 
vary between micrographs as a function of experimental parameters. }
\end{figure}

==> fig_groesdata.tex <==
\begin{figure}
\centering

\hfill
\includegraphics[width=0.13\textwidth]{figs/Phantom.png}
\hfill
\includegraphics[width=0.145\textwidth]{figs/phantomimg0.pdf}
\includegraphics[width=0.145\textwidth]{figs/phantomimg1.pdf}
\includegraphics[width=0.145\textwidth]{figs/phantomimg2.pdf}
\includegraphics[width=0.145\textwidth]{figs/phantomimg3.pdf}
\includegraphics[width=0.145\textwidth]{figs/phantomimg4.pdf}
\hfill
\caption{\label{fig:groesdata}
\marcus{Ali: We need some images like the ones above to put here for GroES}
The structure of GroES (left) and simulated images
(right) generated by choosing orientations and shifts at random,
applying CTFs selected from the thermus dataset and adding noise.
}
\end{figure}

==> fig_initialization.tex <==
\begin{wrapfigure}{r}{0.225\textwidth}
\centering
\includegraphics[width=0.2\textwidth]{figs/Initialization.png}
\caption{\label{fig:initialization}
The random initialization used in all experiments, generated by
summing random spheres.}
\end{wrapfigure}


==> optimization.tex <==
\section{Stochastic Optimization}
\marcus{Here we describe all the different methods we use.}


